Toward Reliable Machine Unlearning: Theory, Algorithms, and Evaluation

We propose new methodologies for both unlearning random set of samples and class unlearning and show that they outperform existing methods. The main driver of our unlearning methods is the similarity of predictions to a retrained model on both the forget and remain samples. We introduce Adversarial Machine UNlearning (AMUN), which surpasses prior state-of-the-art methods for image classification based on SOTA MIA scores. AMUN lowers the model's confidence on forget samples by fine-tuning on their corresponding adversarial examples. Through theoretical analysis, we identify factors governing AMUN's performance, including smoothness. To facilitate training of smooth models with a controlled Lipschitz constant, we propose FastClip, a scalable method that performs layer-wise spectral-norm clipping of affine layers. In a separate study, we show that increased smoothness naturally improves adversarial example transfer, thereby supporting the second factor above. Following the same principles for class unlearning, we show that existing methods fail in replicating a retrained model's behavior by introducing a nearest-neighbor membership inference attack (MIA-NN) that uses the probabilities assigned to neighboring classes to detect unlearned samples and demonstrate the vulnerability of such methods. We then propose a fine-tuning objective that mitigates this leakage by approximating, for forget-class inputs, the distribution over remaining classes that a model retrained from scratch would produce. To construct this approximation, we estimate inter-class similarity and tilt the target model's distribution accordingly. The resulting Tilted ReWeighting(TRW) distribution serves as the desired target during fine-tuning. Across multiple benchmarks, TRW matches or surpasses existing unlearning methods on prior metrics.

==> LOTOS/5.3_prior.tex <==
\subsection{Improving Prior Methods}
\label{subse:prior}


% For training robust ensembles prior methods have proposed different approaches and in this section, we are interested in observing the effect of \texttt{LOTOS} when combined with these prior works to see if the robustness can be further improved. For this purpose, we use TRS~\cite{yang2021trs}, which is one of the SOTA methods in training robust ensembles and is used as the method of choice by recent works~\cite{sitawarin2023defending}. We report the accuracy and robust accuracy of the ensembles against black-box attacks.~\Cref{tab:bn-cifar} shows the results for the ensembles trained with TRS only (TRS), trained with TRS with clipped models (TRS + $C=1$), and trained with both TRS and \texttt{LOTOS} (TRS + \texttt{LOTOS}). As the results show, for both datasets and both model architectures, the robust accuracy of the combined methods is the highest value. This comes at a slight decrease in the accuracy for CIFAR-10 and a more noticeable degradation for CIFAR-100. Note that for this experiment, we did not perform any hyper-parameter tuning and used both methods with the default parameters. For more evaluations on TRS and another SOTA method (DVERGE~\cite{yang2020dverge}), see~\Cref{apx:dverge}.

In this section, we are interested in observing the effectiveness of \texttt{LOTOS} when combined with prior SOTA methods for ensemble robustness.~\Cref{tab:bn-cifar} shows the results for the ensembles trained with TRS~\cite{yang2021trs} only (TRS), trained with TRS with clipped models (TRS + $C=1$), and trained with both TRS and \texttt{LOTOS} (TRS + \texttt{LOTOS}). As the results show, for both datasets and both model architectures, the robust accuracy of the combined methods is the highest value. This comes at a slight decrease in accuracy (more noticeable for CIFAR-100).~\cite{gao2022mora} showed that DVERGE~\cite{yang2020dverge} is more effective than TRS against more elaborate attacks that are specifically designed for ensembles. Hence, we also evaluate the combination of LOTOS with TRS and DVERGE against these attacks to further verify the effectiveness of \texttt{LOTOS} (see~\Cref{apx:dverge}).% for the details and results). 
%For these experiments, we did not perform any hyper-parameter tuning and used all methods with the default parameters. For more evaluations on TRS and another SOTA method. %(DVERGE~\cite{yang2020dverge}), see~\Cref{apx:dverge}.


\begin{table*}[ht!]
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{} l  c c  c  c  c c   @{}}
 \toprule
%\cmidrule(r){1-4}
 
 %\midrule   
 & \multicolumn{3}{@{}c}{\textbf{CIFAR-10}} & \multicolumn{3}{@{}c}{\textbf{CIFAR-100}} \\\addlinespace[0.3em]

   &  TRS & TRS + $C=1$ & TRS + \texttt{LOTOS}
 & TRS & TRS + $C=1$ & TRS + \texttt{LOTOS}  \\\addlinespace[0.3em]

    \cmidrule(r){2-4}
    \cmidrule(r){5-7}

 %& \multicolumn{4}{@{}c}{Accuracy on the test set}   \\ \addlinespace[0.4em]%[0.5ex] 

& \multicolumn{6}{@{}c}{Ensembles of ResNet-18 models}   \\ \addlinespace[0.5em]%[0.5ex] 

 Test Acc & $\bf 94.4 \pm 0.05$ & $94.1 \pm 0.17$ & $92.7 \pm 0.09$
 & $\bf 73.28 \pm 0.46$ & $72.94 \pm 0.29$ & $67.23 \pm 1.22$ \\\addlinespace[0.3em]
 
 Robust Acc & $30.8 \pm 0.65$ & $35.9 \pm 1.35$ & $\bf 41.5 \pm 1.04$  
 & $12.3 \pm 0.53$ & $16.3 \pm 0.57$ & $\bf 20.7 \pm 0.99$ \\\addlinespace[0.3em]

%  Orig & $29.8 \pm 0.43$ & $39.6 \pm 1.29$ & $\bf 42.8 \pm 0.87$  
%  &  $8.5 \pm 0.42$ & $15.2 \pm 0.54$ & $\bf 21.1 \pm 0.63$ \\\addlinespace[0.3em]
% 
%  $C=1.0$ & $31.9 \pm 0.88$ &  $32.1 \pm 1.4$ &  $\bf 40.2 \pm 1.20$ 
%  & $16.2 \pm 0.64$ &  $17.5 \pm 0.60$ &  $\bf 20.2 \pm 1.36$ \\\addlinespace[0.3em]


& \multicolumn{6}{@{}c}{Ensembles of DLA models}   \\ \addlinespace[0.5em]%[0.5ex] 

 Test Acc & $\bf 94.72 \pm 0.06$ & $92.79 \pm 0.13$ & $93.18 \pm 0.14$
 & $\bf 72.6 \pm 0.54$ & $63.3 \pm 1.20$ & $66.8 \pm 1.26$ \\\addlinespace[0.3em]
 
 Robust Acc & $31.2 \pm 0.80$ & $32.9 \pm 0.77$ & $\bf 35.3 \pm 0.39$  
 & $23.2 \pm 0.41$  & $23.7 \pm 2.36$ & $\bf 24.3 \pm 1.67$ \\\addlinespace[0.3em]

%  Orig & $32.2 \pm 0.99$ & $35.1 \pm 0.69$ & $\bf 37.6 \pm 0.23$  
%  & $22.5 \pm 0.66$  & $24.7 \pm 2.36$ & $\bf 25.6 \pm 2.04$ \\\addlinespace[0.3em]
% 
%  $C=1.0$ & $30.1 \pm 0.60$ &  $30.7 \pm 0.85$ &  $\bf 33.0 \pm 0.55$ 
%  & $\bf 23.8 \pm 0.16$ &  $22.6 \pm 2.35$ &  $22.9 \pm 1.31$ \\\addlinespace[0.3em]

   
%\cmidrule(r){1-4}                        
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\caption{\footnotesize {\bf Robust accuracy against black-box attacks in ensembles of ResNet-18 and ensembles of DLA models trained with TRS.} We use ensembles of three models for three different cases; trained with TRS only, trained with TRS while clipping the models, and trained with both TRS and \texttt{LOTOS}. As the results show, using TRS and \texttt{LOTOS} achieves a robust accuracy that is higher than when either of these methods is used.}
\label{tab:bn-cifar}
\vskip -0.2in
\end{table*}




% \begin{table*}[ht!]
% \caption{\footnotesize {\bf Robust accuracy against black-box attacks in ensembles of DLA models trained with TRS (wBN)} with adversarial training formulation for the computation of the norm of the loss. The source models are either original models or clipped models. The target models are ensemble of three DLA models for three different cases; original models, clipped ones, and trained with LOTOS. }
% \label{tab:bn-dla-cifar}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{@{} l  c c  c  c  c c   @{}}
%  \toprule
% %\cmidrule(r){1-4}
%  
%  %\midrule   
%  & \multicolumn{3}{@{}c}{\textbf{CIFAR-10}} & \multicolumn{3}{@{}c}{\textbf{CIFAR-100}} \\\addlinespace[0.3em]
% 
%    &  TRS & TRS-C & TRS-L
%  & TRS & TRS-C & TRS-L  \\\addlinespace[0.3em]
% 
%     \cmidrule(r){2-4}
%     \cmidrule(r){5-7}
% 
%  %& \multicolumn{4}{@{}c}{Accuracy on the test set}   \\ \addlinespace[0.4em]%[0.5ex] 
% 
%  Acc & $\bf 94.72 \pm 0.06$ & $92.79 \pm 0.13$ & $93.18 \pm 0.14$
%  & $\bf 72.6 \pm 0.54$ & $63.3 \pm 1.20$ & $66.8 \pm 1.26$ \\\addlinespace[0.3em]
%  
%  Orig & $32.2 \pm 0.99$ & $35.1 \pm 0.69$ & $\bf 37.6 \pm 0.23$  
%  & $22.5 \pm 0.66$  & $24.7 \pm 2.36$ & $\bf 25.6 \pm 2.04$ \\\addlinespace[0.3em]
% 
%  $C=1.0$ & $30.1 \pm 0.60$ &  $30.7 \pm 0.85$ &  $\bf 33.0 \pm 0.55$ 
%  & $\bf 23.8 \pm 0.16$ &  $22.6 \pm 2.35$ &  $22.9 \pm 1.31$ \\\addlinespace[0.3em]
% 
%    
% %\cmidrule(r){1-4}                        
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}




%\begin{table*}[t!]
%\caption{Transferability rate of black-box attacks to ensembles trained with TRS with adversarial training formulation for the computation of the norm of the loss. The source models are either original models or clipped models. The target models are ensemble of three models for three different cases; original models, clipped ones, and trained with LOTOS. We report the results for both the cases where batch norm layers are removed and the case where they are kept.}
%\label{tab:bn-cifar}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{@{} l  c c  c  c  c c   @{}}
% \toprule
 
% & \multicolumn{3}{@{}c}{\textbf{CIFAR-10}} & \multicolumn{3}{@{}c}{\textbf{CIFAR-100}} \\\addlinespace[0.3em]

%   &  TRS & TRS-C & TRS-L
% & TRS & TRS-C & TRS-L  \\\addlinespace[0.3em]

%    \cmidrule(r){2-4}
%    \cmidrule(r){5-7}

% Acc & $80.7 \pm 1.34$ & $61.0 \pm 0.85$ & $56.2 \pm 1.30$   
% & $73.0 \pm 1.35$ & $61.3 \pm 0.57$ & $60.4 \pm 0.66$  \\\addlinespace[0.3em]
 
% Orig & $80.7 \pm 1.34$ & $61.0 \pm 0.85$ & $56.2 \pm 1.30$   
% & $73.0 \pm 1.35$ & $61.3 \pm 0.57$ & $60.4 \pm 0.66$  \\\addlinespace[0.3em]

% $C=1.0$ & $81.5 \pm 1.32$ & $86.4 \pm 1.09$ & $83.3 \pm 0.87$ 
% & $62.3 \pm 2.22$  & $66.6 \pm 0.80$ &  $65.3 \pm 1.22$ \\\addlinespace[0.3em]
                    
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table*}
